An In-Context Learning Agent for Formal Theorem-Proving

We present an in-context learning agent for formal theorem-proving in environments like Lean and Coq. Current state-of-the-art models for the problem are finetuned on environment-specific proof data. By contrast, our approach, called COPRA, repeatedly asks a high-capacity, general-purpose large language model (GPT-4) to propose tactic applications from within a stateful backtracking search. Proposed tactics are executed in the underlying proof environment. Feedback from the execution is used to build the prompt for the next model query, along with selected information from the search history and lemmas retrieved from an external database. We evaluate our implementation of COPRA on the miniF2F benchmark for Lean and a set of Coq tasks from the CompCert project. On these benchmarks, COPRA significantly outperforms few-shot invocations of GPT-4. It also compares favorably against finetuning-based approaches, outperforming ReProver, a state-of-the-art finetuned approach for Lean, in terms of the pass@1 metric. Our code and data are available at https://github.com/trishullab/copra.

==> lstlean.tex <==
% Listing style definition for the Lean Theorem Prover.
% Defined by Jeremy Avigad, 2015, by modifying Assia Mahboubi's SSR style.
% Unicode replacements taken from Olivier Verdier's unixode.sty

\lstdefinelanguage{lean} {

% Anything betweeen $ becomes LaTeX math mode
mathescape=true,
% Comments may or not include Latex commands
texcl=false,

% keywords, list taken from lean-syntax.el
morekeywords=[1]{
import, prelude, protected, private, noncomputable, definition, meta, renaming,
hiding, exposing, parameter, parameters, begin, conjecture, constant, constants,
hypothesis, lemma, corollary, variable, variables, premise, premises, theory,
print, theorem, proposition, example, abstract,
open, as, export, override, axiom, axioms, inductive, with, without,
structure, record, universe, universes,
alias, help, precedence, reserve, declare_trace, add_key_equivalence,
match, infix, infixl, infixr, notation, postfix, prefix, instance,
eval, vm_eval, check, coercion, end, this, suppose,
using, using_well_founded, namespace, section, fields,
attribute, local, set_option, extends, include, omit, classes, class,
instances, coercions, attributes, raw, replacing,
calc, have, show, suffices, by, in, at, let, forall, Pi, fun,
exists, if, dif, then, else, assume, take, obtain, from, aliases, register_simp_ext,
mutual, def, run_command
},

% Sorts
morekeywords=[2]{Type, Prop, Type*, Type₀, Type₁, Type₂, Type₃},

% tactics, list taken from lean-syntax.el
% morekeywords=[3]{
% Cond, or_else, then, try, when, assumption, eassumption, rapply,
% apply, fapply, eapply, rename, intro, intros, all_goals, fold, focus, focus_at,
% generalize, generalizes, clear, clears, revert, reverts, back, beta, done, exact, rexact,
% refine, repeat, whnf, rotate, rotate_left, rotate_right, inversion, cases, rewrite,
% xrewrite, krewrite, blast, simp, esimp, unfold, change, check_expr, contradiction,
% exfalso, split, existsi, constructor, fconstructor, left, right, injection, congruence, reflexivity,
% symmetry, transitivity, state, induction, induction_using, fail, append,
% substvars, now, with_options, with_attributes, with_attrs, note
% },

% modifiers, taken from lean-syntax.el
% note: 'otherkeywords' is needed because these use a different symbol.
% this command doesn't allow us to specify a number -- they are put with [1]
% otherkeywords={
% [persistent], [notation], [visible], [instance], [trans_instance],
% [class], [parsing-only], [coercion], [unfold_full], [constructor],
% [reducible], [irreducible], [semireducible], [quasireducible], [wf],
% [whnf], [multiple_instances], [none], [decl], [declaration],
% [relation], [symm], [subst], [refl], [trans], [simp], [congr], [unify],
% [backward], [forward], [no_pattern], [begin_end], [tactic], [abbreviation],
% [reducible], [unfold], [alias], [eqv], [intro], [intro!], [elim], [grinder],
% [localrefinfo], [recursor]
% },

% Various symbols
literate=
{α}{{\ensuremath{\mathrm{\alpha}}}}1
{β}{{\ensuremath{\mathrm{\beta}}}}1
{γ}{{\ensuremath{\mathrm{\gamma}}}}1
{δ}{{\ensuremath{\mathrm{\delta}}}}1
{ε}{{\ensuremath{\mathrm{\varepsilon}}}}1
{ζ}{{\ensuremath{\mathrm{\zeta}}}}1
{η}{{\ensuremath{\mathrm{\eta}}}}1
{θ}{{\ensuremath{\mathrm{\theta}}}}1
{ι}{{\ensuremath{\mathrm{\iota}}}}1
{κ}{{\ensuremath{\mathrm{\kappa}}}}1
{μ}{{\ensuremath{\mathrm{\mu}}}}1
{ν}{{\ensuremath{\mathrm{\nu}}}}1
{ξ}{{\ensuremath{\mathrm{\xi}}}}1
{π}{{\ensuremath{\mathrm{\mathnormal{\pi}}}}}1
{ρ}{{\ensuremath{\mathrm{\rho}}}}1
{σ}{{\ensuremath{\mathrm{\sigma}}}}1
{τ}{{\ensuremath{\mathrm{\tau}}}}1
{φ}{{\ensuremath{\mathrm{\varphi}}}}1
{χ}{{\ensuremath{\mathrm{\chi}}}}1
{ψ}{{\ensuremath{\mathrm{\psi}}}}1
{ω}{{\ensuremath{\mathrm{\omega}}}}1

{Γ}{{\ensuremath{\mathrm{\Gamma}}}}1
{Δ}{{\ensuremath{\mathrm{\Delta}}}}1
{Θ}{{\ensuremath{\mathrm{\Theta}}}}1
{Λ}{{\ensuremath{\mathrm{\Lambda}}}}1
{Σ}{{\ensuremath{\mathrm{\Sigma}}}}1
{Φ}{{\ensuremath{\mathrm{\Phi}}}}1
{Ξ}{{\ensuremath{\mathrm{\Xi}}}}1
{Ψ}{{\ensuremath{\mathrm{\Psi}}}}1
{Ω}{{\ensuremath{\mathrm{\Omega}}}}1

{ℵ}{{\ensuremath{\aleph}}}1

{≤}{{\ensuremath{\leq}}}1
{≥}{{\ensuremath{\geq}}}1
{≠}{{\ensuremath{\neq}}}1
{≈}{{\ensuremath{\approx}}}1
{≡}{{\ensuremath{\equiv}}}1
{≃}{{\ensuremath{\simeq}}}1

{≤}{{\ensuremath{\leq}}}1
{≥}{{\ensuremath{\geq}}}1

{∂}{{\ensuremath{\partial}}}1
{∆}{{\ensuremath{\triangle}}}1 % or \laplace?

{∫}{{\ensuremath{\int}}}1
{∑}{{\ensuremath{\mathrm{\Sigma}}}}1
{Π}{{\ensuremath{\mathrm{\Pi}}}}1

{⊥}{{\ensuremath{\perp}}}1
{∞}{{\ensuremath{\infty}}}1
{∂}{{\ensuremath{\partial}}}1

{∓}{{\ensuremath{\mp}}}1
{±}{{\ensuremath{\pm}}}1
{×}{{\ensuremath{\times}}}1

{⊕}{{\ensuremath{\oplus}}}1
{⊗}{{\ensuremath{\otimes}}}1
{⊞}{{\ensuremath{\boxplus}}}1

{∇}{{\ensuremath{\nabla}}}1
{√}{{\ensuremath{\sqrt}}}1

{⬝}{{\ensuremath{\cdot}}}1
{•}{{\ensuremath{\cdot}}}1
{∘}{{\ensuremath{\circ}}}1

%{⁻}{{\ensuremath{^{\textup{\kern1pt\rule{2pt}{0.3pt}\kern-1pt}}}}}1
{⁻}{{\ensuremath{^{-}}}}1
{▸}{{\ensuremath{\blacktriangleright}}}1

{∧}{{\ensuremath{\wedge}}}1
{∨}{{\ensuremath{\vee}}}1
{¬}{{\ensuremath{\neg}}}1
{⊢}{{\ensuremath{\vdash}}}1

%{⟨}{{\ensuremath{\left\langle}}}1
%{⟩}{{\ensuremath{\right\rangle}}}1
{⟨}{{\ensuremath{\langle}}}1
{⟩}{{\ensuremath{\rangle}}}1

{↦}{{\ensuremath{\mapsto}}}1
{→}{{\ensuremath{\rightarrow}}}1
{↔}{{\ensuremath{\leftrightarrow}}}1
{⇒}{{\ensuremath{\Rightarrow}}}1
{⟹}{{\ensuremath{\Longrightarrow}}}1
{⇐}{{\ensuremath{\Leftarrow}}}1
{⟸}{{\ensuremath{\Longleftarrow}}}1

{∩}{{\ensuremath{\cap}}}1
{∪}{{\ensuremath{\cup}}}1
{⊂}{{\ensuremath{\subseteq}}}1
{⊆}{{\ensuremath{\subseteq}}}1
{⊄}{{\ensuremath{\nsubseteq}}}1
{⊈}{{\ensuremath{\nsubseteq}}}1
{⊃}{{\ensuremath{\supseteq}}}1
{⊇}{{\ensuremath{\supseteq}}}1
{⊅}{{\ensuremath{\nsupseteq}}}1
{⊉}{{\ensuremath{\nsupseteq}}}1
{∈}{{\ensuremath{\in}}}1
{∉}{{\ensuremath{\notin}}}1
{∋}{{\ensuremath{\ni}}}1
{∌}{{\ensuremath{\notni}}}1
{∅}{{\ensuremath{\emptyset}}}1

{∖}{{\ensuremath{\setminus}}}1
{†}{{\ensuremath{\dag}}}1

{ℕ}{{\ensuremath{\mathbb{N}}}}1
{ℤ}{{\ensuremath{\mathbb{Z}}}}1
{ℝ}{{\ensuremath{\mathbb{R}}}}1
{ℚ}{{\ensuremath{\mathbb{Q}}}}1
{ℂ}{{\ensuremath{\mathbb{C}}}}1
{⌞}{{\ensuremath{\llcorner}}}1
{⌟}{{\ensuremath{\lrcorner}}}1
{⦃}{{\ensuremath{\{\!|}}}1
{⦄}{{\ensuremath{|\!\}}}}1

{₁}{{\ensuremath{_1}}}1
{₂}{{\ensuremath{_2}}}1
{₃}{{\ensuremath{_3}}}1
{₄}{{\ensuremath{_4}}}1
{₅}{{\ensuremath{_5}}}1
{₆}{{\ensuremath{_6}}}1
{₇}{{\ensuremath{_7}}}1
{₈}{{\ensuremath{_8}}}1
{₉}{{\ensuremath{_9}}}1
{₀}{{\ensuremath{_0}}}1

{¹}{{\ensuremath{^1}}}1

{ₙ}{{\ensuremath{_n}}}1
{ₘ}{{\ensuremath{_m}}}1
{↑}{{\ensuremath{\uparrow}}}1
{↓}{{\ensuremath{\downarrow}}}1

{▸}{{\ensuremath{\triangleright}}}1

{Σ}{{\color{symbolcolor}\ensuremath{\Sigma}}}1
{Π}{{\color{symbolcolor}\ensuremath{\Pi}}}1
{∀}{{\color{symbolcolor}\ensuremath{\forall}}}1
{∃}{{\color{symbolcolor}\ensuremath{\exists}}}1
{λ}{{\color{symbolcolor}\ensuremath{\mathrm{\lambda}}}}1

{:=}{{\color{symbolcolor}:=}}1
{=}{{\color{symbolcolor}=}}1
{<}{{\color{symbolcolor}<}}1
{+}{{\color{symbolcolor}+}}1
{*}{{\color{symbolcolor}*}}1,

% Comments
%comment=[s][\itshape \color{commentcolor}]{/-}{-/},
morecomment=[s][\color{commentcolor}]{/-}{-/},
morecomment=[l][\itshape \color{commentcolor}]{--},

% Spaces are not displayed as a special character
showstringspaces=false,

% keep spaces
keepspaces=true,

% String delimiters
morestring=[b]",
morestring=[d],

% Size of tabulations
tabsize=3,

% Enables ASCII chars 128 to 255
extendedchars=false,

% Case sensitivity
sensitive=true,

% Automatic breaking of long lines
breaklines=true,

% Default style fors listingsred
basicstyle=\ttfamily,

% Position of captions is bottom
captionpos=b,

% Full flexible columns
columns=[l]fullflexible,


% Style for (listings') identifiers
identifierstyle={\ttfamily\color{black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the begining of the
% document. Don't know how to do better.

% Style for declaration keywords
keywordstyle=[1]{\ttfamily\color{keywordcolor}},

% Style for sorts
keywordstyle=[2]{\ttfamily\color{sortcolor}},

% Style for tactics keywords
% keywordstyle=[3]{\ttfamily\color{tacticcolor}},

% Style for attributes
% keywordstyle=[4]{\ttfamily\color{attributecolor}},

% Style for strings
stringstyle=\ttfamily,

% Style for comments
% commentstyle={\ttfamily\footnotesize },

}

==> old_evaluation.tex <==
\newpage
\textbf{OLD: Evaluation section}
Our findings about \copra are that: (i) the approach can find proofs significantly quicker than the state-of-the-art finetuning-based baselines, both in terms of number of LLM queries and wall-clock time;  (ii) in problems where all current methods fail, \copra fails faster; (iii) the use of GPT-4, as opposed to GPT-3.5, within the agent is essential for success; and (iv) backtracking significantly improves the system's performance on harder problems. 
Now we elaborate on our experimental methodology and these results. 

\parag{Benchmarks.} 
We evaluate \copra on two domains: (i) $\minif$ \citep{zheng2021minif2f}, a collection of 244 Lean 3 formalizations of mathematics competition problems, solved using a range of techniques such as induction, algebraic manipulation, and contradiction; and (ii) a set of Coq problems from the CompCert compiler verification project \citep{leroy2009formal} that was previously used to evaluate the \proverbot system \citet{sanchez2020generating}. 

\parag{Implementing \copra.} Our implementation of \copra can have GPT-3.5, GPT-4, GPT-4-turbo \citep{openai2023gpt4turbo} or CodeLlama \citep{roziere2023code} as the underlying LLM and can interact with both the Lean and the Coq proof environments. 
Because of the substantial cost of GPT-4 queries, we cap the number of LLM queries that \copra can make at 60 for most of our experiments.
%To further reduce costs, \system first tries to prove its theorems in a single LLM query (one-shot prompting), and then it invokes the agent behavior when it fails to find a proof via one-shot prompting. 



The Lean version of our system uses BM25 search on the \texttt{mathlib} library for retrieval of relevant lemmas. Inspired by the DSP approach \citep{jiang2022draft}, we also use the informal theorem statements in the $\minif$ dataset to generate informal proofs of theorems using one-shot prompting of the underlying LLM. The prompt has one fixed example (for all invocations) of generating informal proof for a given informal theorem statement. These informal proofs are included as part of the global context (we also consider an ablation where the informal proofs are not used). 

In the Compcert domain, we compare with \proverbot \citep{sanchez2020generating}, which, while not LLM-based, is the best publicly available model for Coq. Unlike $\minif$, this benchmark comes with a large training set as well as a test set, and we use the training set for retrieving relevant lemmas and definitions. Our retrieval mechanism, in this case, is a simple BM25 search. Given that this domain does not come with informal theorem statements, we do not use informal proofs here.

At first, the retrieval mechanism is not used by the agent to keep the prompts smaller and cost-effective, but if the agent fails to find the proofs then retrieval is used to enrich the proof state before prompting the LLM. Similarly, informal proofs in the case of $\minif$ are only used when the agent fails to find the proof with and without retrieval. 
%All the informal proofs are first generated using a separate one-shot prompt, and then \copra simply uses these proofs along with informal theorem statements to enhance its prompts. 
More details about the setup can be found in \Cref{sec:copra-implementation-setup}.

\parag{Baselines.} 
We compare with one-shot invocations of GPT-3.5 and GPT-4 in both the $\minif$ and the Compcert domains. 
The ``system prompt" in the one-shot approach is slightly different than that for \copra, containing instructions to generate a proof in one go rather than step by step. For both \copra and the one-shot baselines, the prompt contains a single proof example that clarifies how proofs need to be formatted. 
This proof example remains the same for all test cases.

\renewcommand\theadfont{}


We also consider an ablation of \copra that uses GPT-3.5 as its LLM and another that does not use backtracking. For the $\minif$ dataset, we also have additional baselines with models like CodeLlama \citep{roziere2023code}, and ablations of \copra's retrieval and use of informal proofs capabilities. As for fine-tuned baselines, a challenge is that all existing open-source theorem-proving systems only target a single proof environment. As a result, we had to choose different baselines for the Lean ($\minif$) and Coq (Compcert) domains. 

Our fine-tuned baseline for the $\minif$ domain is \reprover, a state-of-the-art, retrieval-augmented open-source prover that is part of the Leandojo project \citep{yang2023leandojo}. 
% We use BM25 search on Lean's \texttt{mathlib} library for retrieval of relevant lemmas. We also use the informal theorem statements in the $\minif$ dataset first to generate all the informal proofs using the one-shot prompting of the underlying LLM. The prompt has one fixed example (for all invocations) of generating informal proof for a given informal theorem statement.
In the Compcert domain, we compare with \proverbot \citep{sanchez2020generating}, which, while not LLM-based, is the best publicly available model for Coq. 
%Unlike $\minif$, this benchmark comes with a large training set as well as a test set, and we use the training set for retrieving relevant lemmas and definitions. Our retrieval mechanism, in this case, is a simple BM25 search. 

%We compare our approach against Proverbot9001 \cite{sanchez2020generating}, which is the only available model for comparison on the CompCert dataset. 



For cost reasons, our evaluation for Compcert uses 118 out the 501 theorems used in the original evaluation of \proverbot \cite{sanchez2020generating}. For fairness, we include all the 98 theorems proved by \proverbot in our subset. The remaining theorems are randomly sampled. 



% \begin{table}
% %\begin{wraptable}{l}{3.3in}
% \vspace{-0.1in}
% %\begin{table}[t]
%     \centering
%     {\footnotesize
%     \begin{tabular}{|l | l | l |} 
%  \hline
%  Approach & \thead{\# Theorems\\proved\\/\\\# Theorems}  & \thead{\% \\proved}\\ [0.5ex] 
%  \hline
%  \hline
%  \multicolumn{3}{|c|}{miniF2F Test Dataset} \\
%  \hline
%   \thead{\system (GPT-4-turbo + retrieval) \\w/o backtracking}  & 64/244 & 26.23\% \\
%   \textbf{\system (GPT-4-turbo + retrieval)} & \textbf{65/244} & \textbf{26.64}\% \\
%   \hline
%  \hline
% \multicolumn{3}{|c|}{CompCert Test Dataset} \\
%  \hline
%  \thead{\system (GPT-4-turbo + retrieval) \\w/o backtracking}  & 33/118 & 27.97\% \\
%  \textbf{\system (GPT-4-turbo  + retrieval)} & \textbf{57/118} & \textbf{48.3}\% \\
%  \hline
%  \end{tabular}
%  }
%  \vspace{-0.1in}
% \caption{Ablation showing the effectiveness of backtracking}
% \label{tab:copra-ablation}
% \vspace{-0.1in}
% %\end{wraptable}
% \end{table}


\parag{Metric.}
%pass@$k$-guidance-steps.} 
The standard metric for evaluating theorem-provers is \emph{pass@k} \citep{lample2022hypertree,yang2023leandojo}. In this metric, a prover is given a budget of $k$ 
\emph{proof attempts}; the method is considered successful if one of these attempts leads to success.
However, a key objective of our research is to discover proofs \emph{quickly}, with fewer LLM queries and lower wall-clock time. The pass@k metric does not evaluate this characteristic as it does not quantify the number of LLM queries or the amount of time needed by a proof attempt.   

To address this concern, we introduce a new metric, \emph{pass@k-guidance-steps}, and 
evaluate \copra and its competitors using this metric. Here, we measure the number of correct proofs that a prover can generate with a budget of \emph{$k$ or fewer guidance steps from the LLM or any neural model}.  For LLMs, one guidance step is a single inference query. In our case, we use only a single attempt to prove the theorem, hence \emph{pass@k-guidance-step} is comparable to \emph{pass@1} while also capturing finer details 
 about the efficiency of the approach. One challenge here is that we want this metric to be correlated with the number of correct proofs that the prover produces within a wall-clock time budget; however, the cost of an inference query is proportional to the number of responses generated per query. To maintain the correlation between 
the number of inference queries and wall-clock time, we restrict each inference on LLM to a single response (see \Cref{sec:metric-pass-k-guidance} for more details).


\parag{Results}
\Cref{fig:pass_k_inferences_minif2f} shows our comparison results for the $\minif$ domain.
%\reprover and \copra on the pass@$k$-inferences metric. As we see, 
As we see, \copra outperforms \reprover, completing, within just 60 \rebuttal{guidance steps}, problems that \reprover could not solve even after a thousand \rebuttal{guidance steps}. This is remarkable given that \copra is based on a black-box foundation model and \reprover was fine-tuned for at least a week on a dataset derived from Lean's Mathlib library. For fairness, we ran \reprover multiple times with 16, 32, and 64 (default) as the maximum number of guidance steps per proof step. We obtained the highest success rates for \reprover with 64 guidance steps. %of 15.9\%, 20.1\%, and  22.13\% in the respective cases and took the best for comparison.
Our performance is at par with most of the state-of-the-art approaches for the $\minif$ dataset when measured on \emph{pass@1} metric. The best ensemble with \copra proves 29.92\% of $\minif$ test theorems, which is more than 25.82\% for \llemma-34b, \citep{azerbayev2023llemma}, 26.23\% for \llemma-7b \citep{azerbayev2023llemma}, 26.5\% for \reprover \citep{yang2023leandojo}, 29.6\% for expert iteration \citep{polu2022formal}, and 29.9\% for Thor \citep{jiang2022thor}. It is important to note that all these other methods involve fine-tuning or some form of training on the proof data, while on the other hand our method relies only on in-context learning.



\Cref{fig:pass_k_inferences_compcert} shows a comparison between \copra and \proverbot.
%As with $\minif2f$, we have a comparison against one-shot GPT-4 and GPT-3.5 baselines in Table \ref{tab:gpt-baseline-inferences}.
%\ref{fig:compcert_k_inferences} 


%\begin{figure}

We find that \copra is significantly faster than \proverbot in terms of the number of guidance steps needed. Since we put a cap of 60 guidance steps on \copra, it cannot prove all the theorems that \proverbot eventually proves. However, as shown in the \Cref{fig:pass_k_inferences_compcert}, \copra proves more theorems than \proverbot if only 60 guidance steps are allowed. Specifically, we prove 57 theorems as compared to 54 theorems for \proverbot. An ensemble of \copra (GPT-4-turbo + retrieval) with one-shot (GPT-4-turbo) proves 67 theorems within 60 guidance steps. The one-shot baselines with GPT-4-turbo and GPT-3.5 could prove 36 and 10 theorems respectively.



Aggregate statistics for the two approaches, as well as a comparison with the one-shot GPT-3.5 and GPT-4 baselines \rebuttal{(details of baseline setup are mentioned in \Cref{sec:one-shot-baseline-setup})}, appear in Table \ref{tab:gpt-baseline-inferences}. It is clear from this data that the language-agent approach offers a significant advantage over the one-shot approach. For example, \copra solves more than twice as many problems as the one-shot GPT-4 baseline, which indicates that it does not just rely on GPT-4 recalling the proof from its memory (we discuss this in more detail in \Cref{sec:data-leakage-in-gpt-4}). Also, the use of GPT-4 as opposed to GPT-3.5 seems essential. We also observe that an ensemble of one-shot approaches and \copra works better than either one of them.


We establish the correlation between the number of \rebuttal{guidance steps} needed for a proof and wall-clock time in Table \ref{tab:wall-time-miniF2F} \rebuttal{(more details are discussed in \Cref{sec:metric-pass-k-guidance-vs-wall-clock-time})}. 
Although the average time per \rebuttal{guidance step} is higher for \system, \copra still finds proofs almost 4x faster than \reprover. This can explained by the fact that our search is more effective as it uses 28x fewer \rebuttal{guidance steps} than \reprover. These \rebuttal{guidance} steps not only contain the average time spent on generating responses from LLM but at times have some contribution corresponding to the execution of the tactic on the Lean environment itself. 

%We also perform a failure analysis to demonstrate that our approach knows better when to give up proving the theorem. 


Table \ref{tab:wall-time-miniF2F} also offers data on when the different approaches report failures. 
Since \reprover uses a timeout for all theorems, we also use a timeout of \rebuttal{10 minutes} while considering failures in Table \ref{tab:wall-time-miniF2F}. The data indicates that \copra is comparatively better at giving up when the problem is too hard to solve. We also note that less time is spent per \rebuttal{guidance step} in case of failure for all approaches. The use of a failure dictionary (see \Cref{fig:overview} and \Cref{Algorithm}), enables fast failure which enables the use of an ensemble of strategies (like retrieval and informal proofs) with \copra within the 60 guidance-step cap and 10 minutes timeout.

% One might conclude that executing correct tactics like \texttt{linarith} might take a longer time to simplify the goal by trying out possible simplifications. On the other hand, failures can have some rewrites that can be quickly identified by Lean's type-checker but might look very similar to the distribution tactics on which the model is trained. Another important factor to consider in case of a pass is the time taken to execute every successful tactic again for the whole proof length, on the other hand, failures might happen fairly early in the proof search with very short proof lengths.

We show the impact of ablating the backtracking feature of \copra in Table \ref{tab:copra-ablation}. We note that backtracking has a greater positive impact in the Compcert domain. We hypothesize that this is because the Compcert problems are more complex and 
backtracking helps more when the proofs are longer.

% \begin{figure*}
%   \centering
% \begin{subfigure}{0.5\textwidth}
%   \centering
%     \includegraphics[width=.7\linewidth]{img/miniF2F/main_pass@k_inference.png}
%   \caption{miniF2F test dataset}
%   \label{fig:miniF2F_k_inferences}
% \end{subfigure}%
% \begin{subfigure}{0.5\textwidth}
%   \centering
%   \includegraphics[width=.7\linewidth]{img/compcert/main_pass@60_inferences.png}
%   \caption{CompCert test dataset}
%   \label{fig:compcert_k_inferences}
% \end{subfigure}
% \caption{Comparison between \system (our approach) with other approaches on the prove@k-inferences metric.}
% \label{fig:pass_k_inferences}
% \end{figure*}


%We can see that the average number of inferences used by our approach (\system) is way less than other approaches.



Finally, we offer an analysis of the different categories of $\minif$ problems solved by \copra and \reprover in \Cref{fig:problem-category-miniF2F}.
We see that certain kinds of problems, for example, International Mathematics Olympiad (IMO) problems and theorems that require induction, 
are difficult for all approaches.
However, \Cref{fig:steps-per-category-miniF2F} shows that \system takes fewer steps consistently across various categories of problems in $\minif$.

From our qualitative analysis, there are certain kinds of problems where the language-agent approach seems especially helpful.
For instance, \Cref{fig:appendix-miniF2F-example} shows a problem
%the theorem for which ReProver failed to generate the proof whereas \system was able to come up with the proof. 
in the `algebra' category that \reprover could not solve. More examples of interesting Coq and Lean proofs that \copra found appear in the appendix. 


%\parag{Results: CompCert.}
